Distributed Planning for Rigid Robot Formations with Probabilistic Collision Avoidance

This paper presents a distributed method for robots moving in rigid formations while ensuring probabilistic collision avoidance between the robots. The formation is parametrised through the transformation of a base configuration. The robots map their desired velocities into a corresponding desired change in the formation parameters and apply a consensus step to reach agreement on the desired formation and a constraint satisfaction step to ensure collision avoidance within the formation. The constraint set is found such that the probability of collision remains below an upper bound. The method was demonstrated in a manual teleoperation scenario both in simulation and a real-world experiment.

==> sections/implementation.tex <==
\section{Implementation}

